Embed-Search-Align: DNA Sequence Alignment using Transformer Models

DNA sequence alignment involves assigning short DNA reads to the most probable locations on an extensive reference genome. This process is crucial for various genomic analyses, including variant calling, transcriptomics, and epigenomics. Conventional methods, refined over decades, tackle this challenge in 2 steps: genome indexing followed by efficient search to locate likely positions for given reads. Building on the success of Large Language Models in encoding text into embeddings, where the distance metric captures semantic similarity, recent efforts have explored whether the same Transformer architecture can produce embeddings for DNA sequences. Such models have shown early promise in classifying short DNA sequences, such as detecting coding/non-coding regions, and enhancer, promoter sequences. However, performance at sequence classification tasks does not translate to sequence alignment, where it is necessary to search across the genome to align each read, a significantly longer-range task. We bridge this gap by framing the Sequence Alignment task for Transformer models as an "Embed-Search-Align" task. In this framework, a novel Reference-Free DNA Embedding model generates embeddings of reads and reference fragments, which are projected into a shared vector space where the read-fragment distance is used as a surrogate for alignment. Technical contributions include: (1) Contrastive loss for self-supervised training of DNA sequence representations, facilitating rich reference-free, sequence-level embeddings, and (2) a DNA vector store to enable search across fragments on a global scale. DNA-ESA is 99% accurate when aligning 250-length reads onto a human genome (3gb), rivaling conventional methods such as Bowtie and BWA-Mem. DNA-ESA exceeds the performance of 6 Transformer model baselines such as Nucleotide Transformer, Hyena-DNA, and shows task transfer across chromosomes and species.

==> tables.py/mainres_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t]
% \setlength{\tabcolsep}{0.46em} % Adjust the column separation here
% \centering
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{@{}llccccc@{}}
% \toprule
% \multicolumn{2}{c|}{} &
%   \multicolumn{3}{c|}{\textbf{DNA-ESA (ours)}} &
%   \multicolumn{1}{c|}{\,\,\,\,\,\,\href{https://huggingface.co/zhihan1996/DNABERT-2-117M}{\textit{DB2, mean}}\,\,\,\,\,\, } &
%   \href{https://huggingface.co/LongSafari/hyenadna-small-32k-seqlen}{\textit{HD, max}} \\ \midrule
% \multicolumn{1}{l|}{I} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{c|}{Top-$K$ @ 50 / Chr.} &
%   \multicolumn{1}{c|}{\textit{ER incr.}} &
%   \multicolumn{1}{c|}{\textbf{Best}} &
%   \multicolumn{2}{c}{Top-K @ 50 / Chr.} \\ \midrule
% \multicolumn{7}{c}{$Q_{PH} \in [60,90]$} \\ \midrule
% \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{c|}{98.72} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.22}} &
%   \multicolumn{1}{c|}{\textbf{98.94}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}37.4 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}14.6 ± 1.01 \\
% \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{c|}{98.48} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.20}} &
%   \multicolumn{1}{c|}{\textbf{98.68}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}37.4 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}14.8 ± 1.01 \\
% \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{c|}{98.52} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.24}} &
%   \multicolumn{1}{c|}{\textbf{98.76}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}35.9 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}14.6 ± 1.01 \\
% \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{c|}{98.56} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.30}} &
%   \multicolumn{1}{c|}{\textbf{98.86}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}34.9 ± 1.34} &
%   \cellcolor[HTML]{C0C0C0}14.5 ± 1.01 \\ \midrule
% \multicolumn{7}{c}{$Q_{PH} \in [30,60]$} \\ \midrule
% \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{c|}{98.56} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.28}} &
%   \multicolumn{1}{c|}{\textbf{98.84}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}35.4 ± 1.34} &
%   \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 13.7 ± 0.98} \\
% \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{c|}{98.66 ± 0.00} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.20}} &
%   \multicolumn{1}{c|}{\textbf{98.86}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}37.3 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 14.2 ± 0.99} \\
% \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{c|}{98.82} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.20}} &
%   \multicolumn{1}{c|}{\textbf{99.02}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}36.0 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 13.8 ± 0.98} \\
% \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{l|}{0.01} &
%   \multicolumn{1}{c|}{98.56} &
%   \multicolumn{1}{c|}{{\color[HTML]{009901} + 0.30}} &
%   \multicolumn{1}{c|}{\textbf{98.86}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}36.8 ± 1.35} &
%   \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 13.5 ± 0.98} \\ \bottomrule
% \end{tabular}
% }
% \caption{
% \textbf{Performance of DNA-ESA with respect to baselines:} \textit{(with diversity priors -- see Def.~\ref{sec:diversitypriors})} The performance of DNA-ESA approeaches that of conventional algorithmic and far exceeds the performance of Transformer-DNA baselines, DB2, mean and HD, max (top performing baselines from Fig.~\ref{fig:puretests}). Both DNA-ESA and baselines utilize a dedicated vector store for the entire genome, maintaining a consistent search strategy. For details on $I, D, Q_{PH}, K, d_{SW}$, refer to \textit{Recall/Simulator Configurations}. \textcolor{red}{For a description of Explorative Reiteration (ER), please refer to Sec.~\ref{sec:seqa}}.
% }
% %\caption{\textbf{DNA-ESA vs. Baselines Performance:} DNA-ESA matches conventional approaches like StrobeAlign, Minimap, and BWA-Mem2~\citep{strobealign, bwamem2, minimap}, significantly outperforming Transformer-DNA baselines DB2, mean, and HD, max (refer to Fig.~\ref{fig:puretests}). Both DNA-ESA and baselines utilize a dedicated vector store for the entire genome, maintaining a consistent search strategy. For details on $I, D, Q_{PH}, K, d_{SW}$, refer to \textit{Recall/Simulator Configurations}. (Diversity priors as per Def.~\ref{sec:diversitypriors}).}

% \label{tab:mainres}
% \end{table*}




\begin{table*}[h]
\centering
\begin{tabular}{@{}c|lllll|l@{}}
\toprule
\textbf{Model} & \multicolumn{1}{l|}{\textbf{Settings}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}ART\\ (MiSeqv3)\end{tabular}}} & 


 \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{PacBio CCS}\\($\mu(v^*), \sigma(v^*)$)\end{tabular}}

\\ \midrule
\textbf{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$I,D = 0.01, Q=250$,\\ $d_{SW}=2\%$\end{tabular}} & \multicolumn{1}{l|}{\textit{Search}} & \multicolumn{1}{l|}{{[}10,30{]}} & \multicolumn{1}{l|}{{[}30,60{]}} & {[}60,90{]} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ch2, pbmm2\\ dSW=5\%\end{tabular}} \\ \midrule
\multirow{4}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Transformer \\ Architectures\end{tabular}}} & \multicolumn{1}{l|}{\textit{HD (max)}} & \multicolumn{1}{l|}{\multirow{3}{*}{K=50}} & \multicolumn{1}{l|}{13.20 $\pm$ 1.81} & \multicolumn{1}{l|}{17.01 $\pm$ 2.01} & 18.03 $\pm$ 2.05 & \multicolumn{1}{c}{-} \\ \cmidrule(lr){2-2} \cmidrule(l){4-7} 
 & \multicolumn{1}{l|}{\textit{DB2 (mean)}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{30.21 $\pm$ 2.44} & \multicolumn{1}{l|}{39.19 $\pm$ 2.58} & 39.20 $\pm$ 2.58 & \multicolumn{1}{c}{-} \\ \cmidrule(lr){2-2} \cmidrule(l){4-7} 
 & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}DNA-ESA\\ (ours)\end{tabular}}}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{98.40 $\pm$ 0.71} & \multicolumn{1}{l|}{98.64 $\pm$ 0.67} & 98.60 $\pm$ 0.67 & \multicolumn{1}{c}{97.5 $\pm$ 0.82}\\ \cmidrule(l){3-7} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{K=75} & \multicolumn{1}{l|}{\textbf{98.80 $\pm$ 0.62}} & \multicolumn{1}{l|}{\textbf{99.28 $\pm$ 0.52}} & \textbf{98.88 $\pm$ 0.60} & 
 
 \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{97.5 $\pm$ 0.82}\\ (-498.0, 3.78)\end{tabular}}
 
  
 
 
 
 \\ \midrule
\textit{\begin{tabular}[c]{@{}c@{}}Bowtie-2 \\ (Classical)\end{tabular}} & \multicolumn{2}{c|}{-} & \multicolumn{3}{c|}{99.80 $\pm$ 0.19} & 

 \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}99.50$\pm$0.43\\ (-497.9, 3.78)\end{tabular}}
  


\\ \midrule
\textit{diff.} & \multicolumn{2}{c|}{-} & \multicolumn{3}{c|}{\textless{}1\%} & \multicolumn{1}{c}{\textless{}2\%} \\ \bottomrule
\end{tabular}
\vspace{1em}
\caption{
\textbf{Performance of DNA-ESA with respect to baselines:} The performance of DNA-ESA is compared to the DNA-BERT 2 and Hyena-DNA Transformer-based baseline models (with no additional finetuning) -- the top performing baselines from Fig.~\ref{fig:puretests}. In addition, DNA-ESA is also compared with Bowtie-2~\cite{bowtie}, a classical aligner. Comparisons are conducted across varying qualities (\textit{Phred score}) of reads generated by ART~\cite{huang_art_2012}.  Additionally, an external PacBio CCS dataset of ($Q=250$ length-) reads from Chr. 2 of the Ashkenazim Trio - Son sample (as determined by pbmm2~\cite{minimap}) are aligned using both Bowtie-2 and DNA-ESA. All baseline models utilize a dedicated vector store. For details on $I, D, Q_{PH}, K, d_{SW}$, refer to \textit{Recall/Simulator Configurations}. Across models and ART-generated datasets, the performance of DNA-ESA supersedes other Transformer-based models and is comparable to Bowtie-2 to within $1\%$. With respect to reads from PacBio CCS, DNA-ESA performs with $2\%$ of Bowtie-2 after controlling for the  intrinsic quality of retrieved fragments according to the SW distance. Mean ($\mu$) and standard deviation ($\sigma$) across the top SW distance values ($v^*$) of reads successfully aligned in the case of DNA-ESA and Bowtie-2 models are reported).
}
\label{tab:mainres}
\end{table*}

==> tables.py/noisy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\small\addtolength{\tabcolsep}{-3pt}
\centering
\begin{tabular}{@{}l|cccc|ccc@{}}
\toprule
                  & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}MiSeqv3 - Q = 250\\ (via ART, PH in {[}10,20{]}, I,D:1\%)\end{tabular}}                                                                                                                                                                                                                                                                         & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}PacBio, CCS - pbmm2, chr2\\ (Ashkenazim Trio, Son)\end{tabular}}                  \\ \midrule \midrule
\textbf{Model}    & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Very-high \\ Sensitivity\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Alignment\\ SW (500)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Very-high \\ Specificity\end{tabular}}}      & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Alignment\\ SW (500)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Q=250}}       & \multicolumn{1}{c|}{\textbf{Q=350}}       & \textbf{Q=500}                            \\ \midrule 
\textit{Bowtie-2} & \multicolumn{1}{c|}{\textbf{\textgreater{}99.9}}                                               & \multicolumn{1}{c|}{490.2}                                                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}87.0 ± 0.94\\ (--mp 1000 \\ --np 1000)\end{tabular}} & 490.4                                                                                      & \multicolumn{1}{c|}{\textless +2.0\%}     & \multicolumn{1}{c|}{\textless +2.8\%}     & \textless +2.5\%                          \\ \midrule
\textbf{DNA-ESA}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}94.4 ± 0.60\\ (dSW=30)\end{tabular}}            & \multicolumn{1}{c|}{488.3}                                                                 & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}89.0 ± 0.87\\ (@dSW=15)\end{tabular}}}       & \textbf{490.6}                                                                             & \multicolumn{1}{c|}{\textbf{97.5 ± 0.47}} & \multicolumn{1}{c|}{\textbf{96.5 ± 0.55}} & \multicolumn{1}{l}{\textbf{97.0 ± 0.51}} \\ \bottomrule
\end{tabular}
\caption{\textbf{DNA-ESA performance on noisy reads:} Noisy reads are simulated using ART ($Q_{PH} = 20$, $I,D=1\%$) and derived from an external PacBio CCS read dump available in GIAB. The reads from PacBio are filtered to those derived from Chr. 2 as determined using the pbmm package~\cite{minimap}. In this evalaution, DNA-ESA is contextualized with Bowtie-2~\cite{bowtie}, a popular conventional alignment tool. On both datasets, DNA-ESA performs slightly worse than Bowtie-2. Despite this, the quality of the retrieved fragments -- as measured using the SW distance -- is very similar. Note that in all cases, the performance of DNA-ESA is comparable (within $1\%$) to those reported in Table.~\ref{tab:mainres}.}
\label{tab:highnoise}
\end{table*}

==> tables.py/sweep.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|lll|lll|lll|}
\hline
\multicolumn{1}{|l|}{top-K} &
  \multicolumn{1}{l|}{I} &
  D &
  \multicolumn{3}{l|}{Recall @ QPH in 30 to 60} &
  \multicolumn{3}{l|}{Recall @ QPH in 30 to 60} \\ \hline
\multicolumn{3}{|l|}{} &
  \multicolumn{1}{l|}{Exact} &
  \multicolumn{1}{l|}{d SW \textless{}5} &
  d SW \textless{}10 &
  \multicolumn{1}{l|}{Exact} &
  \multicolumn{1}{l|}{d SW \textless{}5} &
  d SW \textless{}10 \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{@50}} &
  \multicolumn{1}{l|}{\multirow{2}{*}{0}} &
  0 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{3-9} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{l|}{} &
  0.01 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{2-9} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{l|}{\multirow{2}{*}{0.01}} &
  0 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{3-9} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{l|}{} &
  0.01 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{@100}} &
  \multicolumn{1}{l|}{\multirow{2}{*}{0.00}} &
  0 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{3-9} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  0.01 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{2-9} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\multirow{2}{*}{0.01}} &
  0 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \cline{3-9} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  0.01 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \hline
\end{tabular}
\end{table}
